Learning to Predict Graphs with Fused Gromov-Wasserstein Barycenters

This paper introduces a novel and generic framework to solve the flagship task of supervised labeled graph prediction by leveraging Optimal Transport tools. We formulate the problem as regression with the Fused Gromov-Wasserstein (FGW) loss and propose a predictive model relying on a FGW barycenter whose weights depend on inputs. First we introduce a non-parametric estimator based on kernel ridge regression for which theoretical results such as consistency and excess risk bound are proved. Next we propose an interpretable parametric model where the barycenter weights are modeled with a neural network and the graphs on which the FGW barycenter is calculated are additionally learned. Numerical experiments show the strength of the method and its ability to interpolate in the labeled graph space on simulated data and on a difficult metabolic identification problem where it can reach very good performance with very little engineering.

==> sections/method.tex <==
In Section \ref{subsec:method}, we present a novel model for supervised graph prediction. In Section \ref{subsec:nonparam}, we present a nonparametric method to train the proposed model. In Section \ref{subsec:nns}, we propose a neural networks method to train the proposed model.

\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\textwidth]{figures/illu_fgwbary_nns.pdf}}
\caption{Proposed supervised graph prediction model.}
\label{fig:model2}
\end{center}
\vskip -0.2in
\end{figure*}

\subsection{Proposed model}

\paragraph{Gromov-Wasserstein distance. }\label{subsec:method} Unlabeled
graphs defined by their adjacency matrix $C$ can be represented as a probability
distribution by equipping the nodes with weights $(h_i)_i$ such that $\sum_i h_i=1$
\cite{peyre2016gromov}. These weights indicate the relative importance of the
vertices in the graph. In this work, we do not have access to such information
from unlabeled graphs datasets, and take uniform weights $h_i$ for
all graphs. This way, one can define the Gromov-Wasserstein distance between two
graphs $z_1 = C_1 \in \R^{n_1 \times n_1}$ and $z_2 = C_2 \in \R^{n_2 \times
n_2}$:
\begin{align}
    GW^2_2(z_1, z_2) = \min\limits_{\pi \in \Pi} \sum_{i,j,k,l} (C_1(i,k) - C_2(j,l))^2 \pi_{i,j}\pi_{k,l}
\end{align}
where $\Pi = \{ \pi \in \R^{n_1 \times n_2}_+ | \pi\mathds{1}_{n_{2}} = n_{1}^{-1}\mathds{1}_{n_{1}}, \pi^T\mathds{1}_{n_1}=n_{2}^{-1}\mathds{1}_{n_{2}}\}$, $\mathds{1}_{n}$ is the all-ones vector with size $n$.


One very interesting property of this divergence is that it allows to
compare unlabeled graphs with potentially different number of nodes. Moreover,
$GW_2$ is symmetric, positive and satisfies the triangle inequality. Furthermore, it
is equal to zero when $z_1$ and $z_2$ are isomorphic, namely when there exist a
bijection $\phi:  \llbracket 1, n_1 \rrbracket \rightarrow \llbracket 1, n_2
\rrbracket$ such that $C_2(\phi(i), \phi(j)) = C_1(i, j)$ for all $i, j \in
\llbracket 1, n_1 \rrbracket$. GW provides a distance on the unlabeled graph
quotiented by the isomorphisms. Hence, it is a natural metric when comparing
graphs, as  in real-world problems, one wants to consider isomorphic graphs as
equal.
\begin{remark} \fl{elaborate on this}
Furthermore, it avoids computing fixed-dimensional feature vector
representations, e.g. encoding which substructures are present in a graph.
\end{remark}

\paragraph{Fused Gromov-Wasserstein distance. } When considering two labeled graphs $z_1 = (C_1, F_1)$ and $z_2 = (C_2, F_2)$, \citet{vayer2020fused} proposed the following combined discrepancy, for a trade-off parameter $\alpha \in [0,1]$:
\begin{equation}\label{eq:fgw}
    \begin{split}
        FGW^2_2((z_1, z_2) =& \min\limits_{\pi \in \Pi(h,g)} \sum_{i,j,k,l} \big[(1-\alpha)\|F_1(i) - F_2(j)\|_{\R^d}^2\\ 
   &+ \alpha (C_1(i,k) - C_2(j,l))^2\big] \pi_{i,j}\pi_{k,l}
    \end{split}
\end{equation}
The optimal transport plan matches the vertices of the two graphs by trying to
minimize the discrepancy between the labels, while preserving the pairwise
similarities between the nodes. Note that FGW distance adapts to the graph space at hand through the choice of the labels' representations $\mathcal{F}$.

\paragraph{Graph prediction with conditional GW barycenters.} 

In this work,
we propose  to use FGW as structured loss $\Delta$, namely we want to
find the function $f_\theta$ minimizing the following expected risk \fl{where are the data, where is the supervised learning problem, m never defined, observed data = supervised learning, never defined}
\begin{align}\label{eq:objective}
    \mathcal{R}_{FGW}(f_\theta) = \E_{x,z}[FGW_2^2(z, f_\theta(x)].
\end{align}
 where the structured prediction model $f_\theta(x)$ can be expressed as a conditional GW barycenter
\begin{align}\label{eq:fgw_estimator}
    f_\theta(x) = \argmin_{z \in \bmZ} \sum_{i=1}^m \alpha_i(x; W) FGW^2_2(z, \bar z_i).
\end{align}
where $\alpha_i(x; W): \bmX \rightarrow \R$ are weight functions which can be
understood as a similarity scores between $x$ and $x_i$. Note that depending on
the estimator we want to learn the parameters $\theta$ of $f_\theta$ can be only
the parameters $\theta=W$ of the conditional weight estimator $\alpha_W$  or
 the parameter $\theta=(W, \bar z_i, \forall i)$ for the conditional weights and the template graphs $\bar z_i$. \fl{what is a template graph?} We denote $(\bar \pi_i)_i$ the $m$ optimal transport plans involved in Equation \eqref{eq:fgw_estimator}.

The proposed model $f_{\theta}$ interpolates in graph space by using the Fr\'echet mean with respect to the FGW distance. It inherits from the good properties of FGW, including, for instance, the invariance under isomorphism (two isomorphic graphs have
equal scores in Eq. \ref{eq:fgw_estimator}). In terms of computation, the proposed model leverages the recent advances in computational optimal transport making the NP-hard computation of the argmin over the space of graph approximately tractable.

\paragraph{Properties of the structure predictor $f_\theta$}
\fl{can you be more precise:  we should highlight clearly that graphs may have not the same size and we are able to deal with it - this is not a fixed size representation, meaning that in the implementation you deal with that, do you ?}
First discuss the shape of the recovered objects by looking at the
solutions of FGW barycenters  \citet[Eq. 14]{peyre2016gromov}
\begin{equation}\label{eq:C}
C(x;W) = n_{out}^2\sum_{i=1}^m \alpha_i(x;W) \bar \pi_k^T\bar C_k\bar \pi_k
\end{equation}
and the feature barycenter \citet[Eq. 8]{cuturi2014fast} 
\begin{equation}\label{eq:A}
    F(x;W) = n_{out}\sum_{i=1}^m \alpha_i(x;W)\bar  F_k \bar \pi_k^T
\end{equation}
The $(\bar\pi_k)_k$ are the optimal transport plans from $(\bar C_k, \bar F_k)_k$ to the
barycenter $(C(x;W), F(x;W))$, and thus depend on $W$. Note that a very
surprising aspect of using FGW barycenter is that the number of nodes
$n_{out}$ is actually not fixed but can be chosen by
the user. Which means that a unique trained model can predict several objects
with a different resolution, allowing potential interoperability at small
resolution and finer modeling at higher resolution. This will be illustrated in
the experimental section.




% \paragraph{Gromov-Wasserstein loss.} 


% In order to solve the learning problem, depending on the problem at hand, we propose two strategies to train the Gromov-Wasserstein barycentric model proposed in Equation \eqref{eq:fgw_estimator}.

\subsection{Nonparametric model}\label{subsec:nonparam}

\rf{RF: gimme some more details here. Do we evaluate this model in teh experiments? how will we do that? I have a hard time believing that the $\alpha_i$ are on the silplex for  dkernel ridge? this should be discussed (basically they can be divided by their sum and yield the same barycenter so it is nota problem but it should be discussed.)}

\fl{first say that you are not learning the templates and you use the training data, then we need to explain this closed-form solution - Note that there pre-exists another reason that the general one (ILE) if the size of C and F were constant, you could define matrix-valued kernel (separable with identity) and could retrieve this form from the close form solution obtained using representer theorem. A nice remark}

Defining a positive definite kernel on the input space $k: \bmX \times \bmX \rightarrow \R$, one can consider the weights of kernel ridge estimation as in \citep{ciliberto2020general}, namely, if $(x_i, z_i)_{i=1}^n$ is the training set, 
\begin{align}\label{eq:krr_weights}
    \alpha(x) = (K_x + n\lambda I_{\R^{n \times n}})^{-1}(k(x, x_1), \dots, k(x, x_n)) \in \R^n
\end{align}
\fl{do not in this paper use the notation $K_x$ and use $k_x$ as the column vector $(k(x,x_1)..k(x,x_n))$.}
with $K_x = (k(x_i, x_j))_{ij} \in \R^{n \times n}$.

The resulting estimator enjoys strong theoretical guarantees as shown in Section \ref{sec:theory}.
\fl{Consistency and excess-risk bounds hold for the non-parametric approach only}
\subsection{Neural networks model}\label{subsec:nns}

In this section the weight functions $\alpha_i$ are instantiated \fl{implemented} with neural networks. We consider the following empirical risk as training objective:
\begin{align}
    \hat R(W) = \frac{1}{n} \sum_{i=1}^n FGW(f(x_i;W), z_i)
\end{align}
Recall that we denoted $(\bar \pi_i)_{i=1}^m$ the $m$ transport plans involved in the model $f(x;W)$. We note $(\pi_i)_{i=1}^n$ the $n$ transport plans involved in the training objective $\hat R(W)$.

In order to optimize $W$, we repeat the following two steps:
\begin{enumerate}
    \item Compute $FGW(f(x_i;W), z_i)$.
    \item Gradient step w.r.t $W$ with fixed $(\tau_k)_k$.
\end{enumerate}

Observe from Equations \eqref{eq:C} and \eqref{eq:A} that step 2 is a bilevel
optimization problem, as the model depends on the $(\bar \pi_i)_i$ that depend on $W$
through the FGW barycenter optimization problem. We take in practice a
subgradient of $\bar \pi_i(W)$ as $0$ since the Quadratic program is non-smooth non
convex but one can suppose that a small change in $C$ will not change the
solution that will be with high probability on a border of the polytope. This
actually corresponds in Pytorch notation to detach the OT plan with respect to the input
which is done by default in POT toolbox. 
This boils down computing the gradient of $\hat R(W)$ with fixed (optimal)
$(\bar \pi_i)_i$. Step 2 is finally a quadratic
program w.r.t $f(x;W) = (C(x;W), F(x;W))$ (See Equation \eqref{eq:fgw}).

We propose various strategies for choosing the templates $(\bar z_i)_i$ in the nonparametric setting. They can be fixed by experts. They can be drawn randomly from the training data, or from $\bmZ'$. They can be learned by minimizing $\hat R$. This leads to an optional training step 3: a gradient step w.r.t the $(\bar z_i)_i$. Notice that it corresponds to a quadratic program w.r.t the $(\bar C_i, \bar F_i)_i$.

\begin{remark}[Model interpretability.] The proposed method has interesting interpretability properties. For a given input $x$, the predicted graph is the Fréchet mean w.r.t the FGW distance, according to the weights $\alpha_i(x)$ and the templates $(\bar z_i)_{i=1}^m$.
\end{remark}


% \begin{remark}[Choice of $n_{out}$.] When computing the output graph with our model, a number of nodes $n_{nodes}$ have to be chosen. In particular, one can compute several graphs with various number of nodes, which is an interesting feature. $n_{nodes}$ can also be predicted from $x$, training a classifier on the same training set, or using $\lfloor \sum_{i=1}^m \alpha_i(x; W) n_{nodes}(z_i)
% \rfloor$.
% \end{remark}



==> sections/structured-pred.tex <==
Let $\bmX$ be the input space and $\bmZ$ be a (representation) space of structured objects which serves as the output space. Structured prediction refers to the following supervised learning task.
Let $\Delta: \bmZ \times \bmZ \rightarrow \R$ be a loss function. Given a finite sample $(x_i, y_i)_{i=1}^N$ independently drawn from an unknown distribution $\rho$ on $\bmX \times \bmZ$, we consider the problem of estimating a target function $f^*: \bmX \rightarrow \bmZ$ with values in the structured objects $\bmZ$ that minimizes the expected risk:
\begin{equation}\label{eq:exp_structured_risk}
    \risk_{\Delta}(f) = \E_{\rho}[\Delta(f(X), Z)],
\end{equation}
by an estimate $\hat{f}$ obtained by minimizing the empirical counterpart of the true risk, namely the empirical risk:~$\emprisk_{\Delta}(f) = \sum_{i=1}^N \Delta(f(x_i), z_i)$.\\

Compared to regression and
multi-classification, a first major challenge usually comes from the nature of $\bmZ$ that may
be finite with a extremely large number of possible of outputs. This makes
the inference (prediction) problem itself combinatorial and hardly tractable. 
A second challenge is that objects of $\bmZ$ may have different sizes requiring to
adapt the size of the output to the input. Finally, $\bmZ$ usually does not
enjoy a vector space properties nor metric properties. %\\
%To address the first challenge, the choice of output data representation as well as the loss function therefore takes on special significance as reflected in the abundant literature on the topic.
\begin{example}
In Supervised Metabolite Identification \citep{heinonen2012,brouard2016fast}, metabolites are to be predicted from the observation of input mass spectra. The set of metabolites candidates is finite and metabolites are molecules of different size, i.e. contain different number of atoms.
\end{example}
To tackle the various challenges of structured prediction, the abundant literature on the topic has mainly explored three directions: energy-based models, surrogate approaches and end-to-end learning. In energy-based models \citep{tsochantaridis2005large,belanger2016structured}, predictions are obtained by maximizing a score function for input-output pairs over the output space. In surrogate approaches \citep{ciliberto2016consistent}, a coding function is used to embed the structured outputs. After minimizing a surrogate loss a decoding procedure is used to map back the surrogate solution.\cb{Add a sentence on end-to-end learning}
\rf{\paragraph{Structured prediction with a score function. } Two } main difficulty appears when one
aims at predicting structured outputs: modeling and computation
\citep{ciliberto2020general}. One needs to design an hypothesis space
$\mathcal{F}$ of functions from $\bmX$ to a non-linear structured space $\bmZ$.
Many methods use models of the form 
\begin{equation}
    f_\theta(x) = \argmax_{z \in \bmZ} F_\theta(x,z)
    \label{eq:structure_pred_model}
\end{equation}
with $F: \bmX \times \bmZ \rightarrow \R$, ensuring $\hat z \in \bmZ$ \fl{avoid using F for different objects}
\citep{weston2002kernel, belanger2016structured, brouard2016input,
ciliberto2020general}. When $\bmZ$ is very big, training $F$ through the argmin
is challenging. Note that the computation of $f_{\theta}(x)$ is not tractable in
general, as optimization in graph space (large and discrete space) is very
difficult, gradient search is unavailable. 
